Mind Your Credit: Assessing the Health of the Ripple Credit Network

The Ripple credit network has emerged as a payment backbone with key advantages for financial institutions and the remittance industry. Its path-based IOweYou (IOU) settlements across different (crypto)currencies conceptually distinguishes the Ripple blockchain from cryptocurrencies, and makes it highly suitable to an orthogonal yet vast set of applications in the remittance world for cross-border transactions and beyond. This work studies the structure and evolution of the Ripple network since its inception, and investigates its vulnerability to devilry attacks that affect the credit of linnet users' wallets. We find that about 13M USD are at risk in the current Ripple network due to inappropriate configuration of the rippling flag on credit links, facilitating undesired redistribution of credit across those links. Although the Ripple network has grown around a few highly connected hub (gateway) wallets that constitute the network's core and provide high liquidity to users, such a credit link distribution results in a user base of around 112,000 wallets that can be financially isolated by as few as 10 highly connected gateway wallets. Indeed, today about 4.9M USD cannot be withdrawn by their owners from the Ripple network due to PayRoutes, a gateway tagged as faulty by the Ripple community. Finally, we observe that stale exchange offers pose a real problem, and exchanges (market makers) have not always been vigilant about periodically updating their exchange offers according to current real-world exchange rates. For example, stale offers were used by 84 Ripple wallets to gain more than 4.5M USD from mid-July to mid-August 2017. Our findings should prompt the Ripple community to improve the health of the network by educating its users on increasing their connectivity, and by appropriately maintaining the credit limits, rippling flags, and exchange offers on their credit links.

==> abstract-copy.tex <==
% !TEX root = main.tex



The Ripple credit network has emerged as a payment backbone with key advantages for financial institutions and the remittance industry. Its path-based IOweYou (IOU) settlements across different (crypto)currencies conceptually distinguishes the Ripple blockchain from cryptocurrencies (such as Bitcoin and altcoins), and makes it highly suitable to an orthogonal yet vast set of applications in the remittance world for cross-border transactions and beyond.

This work studies the structure and evolution of the Ripple network since its inception, and investigates its vulnerability to devilry attacks that affect the IOU credit of linnet users'  wallets.  We find that about 13M USD are at risk in the current Ripple network due to inappropriate configuration of the rippling flag on credit links, facilitating undesired redistribution of credit across those links. Although the Ripple network has grown around a few highly connected hub (gateway) wallets that constitute the core of the network and provide high liquidity to users, such a credit link distribution results in a user base of around 112,000 wallets that can be financially isolated by as few as 10 highly connected gateway wallets. Indeed, today about 4.9M USD cannot be withdrawn by their owners from the Ripple network due to PayRoutes, a gateway tagged as faulty by the Ripple community. Finally, we observe that stale exchange offers pose a real problem, and exchanges (market makers) have not always been vigilant about periodically updating their exchange offers according to current real-world exchange rates. For example, stale offers were used by 84 Ripple wallets to gain more than 4.5M USD from mid-July to mid-August 2017. Our findings should prompt the Ripple community to improve the health of the network by educating its users on increasing their connectivity, and by appropriately maintaining the credit limits, rippling flags, and exchange offers on their IOU credit links.





==> abstract-without-macros.tex <==
% !TEX root = main.tex

\begin{abstract}
Initially proposed as part of the cypherpunk-esque rebellion started by Bitcoin, the Ripple credit network is dramatically reshaping the financial and remittance industries. At its core, the Ripple network is a weighted directed graph of IOweYou credit links, where a transaction between two nodes is only allowed if there is sufficient max-flow between them. These path-based settlements set Ripple apart from the cryptocurrency space (such as Bitcoin and altcoins) both conceptually and in terms of applicability. This work takes an in-depth look at the Ripple network since its inception  in order to understand its structure, evolution, and vulnerability to attacks.
%In particular, we characterize the network graph, its mixing time and the structure and evolution of its communities. 
%We additionally study the security and resilience of the \nw by assessing users' vulnerability to the inherently-allowed 
%transitive nature of path-based transactions and to the disruption caused by nodes in the core of the network. 

We observe that gateway nodes determine not only the graph structure 
but also the existence of clear geographical communities. 
From the security point of view, 
although the core of the network is well-connected and provides high liquidity to \users, 
there is a user base of around $50,000$ \accs prone to disruption 
by as few as $10$ highly connected \accs.
%being then unable to transact their about $14$M USD credit. 
Finally, %we observe that 
we find that %the in principle innocuous 
redistribution of credit (i.e., rippling) among \links as a result of a \tx puts at risk around $30$M USD in the current 
\nw. 
%A correct setup of the balance and limit of \links may mitigate this problem.
%These users must add \links to other nodes and set them with correct balances and limits.
Our study should serve as a wake-up call to inattentive users to improve their connectivity to the network,
and ensure that their rippling flags 
and credit limits on the links are correctly set.

\end{abstract}

==> community-discussion.tex <==
\section{Community-discussion}






==> currency-graphs.tex <==
% !TEX root = main.tex

%\pparagraph{Currency-specific \Resil} 
%%The \links in the \nw can be associated with any currency, even user-defined currencies. 
%At this point, we study whether the \resil for the \nw 
%still holds when considering only \links associated with the top five fiat currencies (i.e., \set{USD, CNY, BTC, JPY, EUR}). 
%For that,  we extract from \mg{2016} the subgraph containing only \links 
%associated with the top five fiat currencies, and calculate its largest connected component. We denote 
%the extracted graph as \cmgraph{2016}. We sort the \accs in \cmgraph{2016} 
%by their degree in decreasing order and pick the top 100. We denote this set as \scurnodes. 
%Finally, we compute the \resilfactor 
%as aforementioned on input \cmgraph{2016} and \scurnodes. 
%The \resilfactor remains in the range (0.5, 0.6) and the \nw can be similarly divided in two main groups as 
%explained above. 

%\section{Analysis of Currency Graphs}
%\label{sec:currency-graphs}
%
%\paragraph{Objective}
%We study the robustness of the prominent currency graphs of Ripple network to failures of nodes in the network. \TODOR{Why to study this? 
%why is different from the previous experiment? What is the importance?}
%
%%\begin{figure*}
%%\centering
%%\begin{subfigure}{\columnwidth}
%%\centering
%%\includegraphics[height=\columnwidth, angle=270]{figures/damagefunctionnum.pdf}
%%\caption{Number of components generated.\label{fig:NetworkRobustness-two}}
%%\end{subfigure}
%%\begin{subfigure}{0.5\textwidth}
%%\centering
%%\includegraphics[height=\columnwidth, angle=270]{figures/damagefunctionsize.pdf}
%%\caption{Size of the biggest component.\label{fig:NetworkRobustness}}
%%\end{subfigure}
%%\caption{Currency graphs' robustness}
%%\end{figure*}
%
%\paragraph{Methodology}
%\TODOR{Write step by step. It might be clearer.}
%For this experiment, we consider our Ripple network as an undirected graph and biggest component of each of five different currency graphs; one per each prominent currency. i.e, USD, BTC, CNY, EUR and JPY. We create one more graph by merging all of these five currency graphs (say "composite graph"). 
%
%We remove nodes from this composite graph one by one without replacement according to the strategies mentioned in the section 7.
%We also capture the metrics like ``number of components generated after removing each node", and ``size of the biggest component" for each approach. 


==> fast-mixing.tex <==
% !TEX root = main.tex

%\Cref{fig:mixing-time} shows that for a fixed mixing time of 100, the variation distance decreases from 0.12 to 0.06 as we prune the \nw to obtain the skeleton. Though this boost in mixing time only occurs after a significant reduction of the network, it is justified to do so as these nodes are not connected to service?\TODON{Please check the statement!!}
%
%We conclude that the \nw is slow-mixing. We also observe that the average mixing time of \nw is higher than the worst case mixing time.
%\TODON{add conclusions}

%\begin{figure}
%\centering
%\begin{subfigure}{.5\columnwidth}
%  \centering
% \includegraphics[height=\columnwidth, angle=270]{images/mixing-lb.eps}
%  \caption{Lower Bound}
%  \label{figure:mt}
%\end{subfigure}%
%\begin{subfigure}{.5\columnwidth}
%  \centering
%  \includegraphics[height=\columnwidth, angle=270]{images/mixing-avg.eps}
%  \caption{Average Mixing Time}
%  \label{figure:mt-avg}
%\end{subfigure}
%\caption{Lower Bound Vs Average Mixing Time for \nw and Skeleton Network}
%\TODOA{too small fonts. All figures should use same/similar fonts, line widths, no grid etc}
%\label{figure:mixing-time}
%\end{figure}
%\TODOP{I think the content below might not be really needed}

%\paragraph{Objective}
%To estimate the nature of mixing time of the Ripple network \TODON{Add more...}
%
%\paragraph{Description}
%Mixing time refers to how quickly a random walk converges to a stationary distribution. To calculate the mixing time, we first need to understand some ideas of random walk over a graph. 
%
%A random walk over a graph is represented by a Markov chain, which essentially captures this process of moving from one node to another in the graph\cite{}. A Random walk R of length k over a graph G is defined as sequence of vertices starting from an initial node and ending at a final node, following the transition probability defined in \ref{eqn:mt}. For an erdogic Markov chain (i.e. irreducible and aperiodic), we have a unique stationary distribution $\pi$ and as $k\rightarrow\infty$, the distribution for random walk converges to $\pi$. Stationary distribution is a probability distribution which is invariant to transition matrix (${\pi}P = \pi$). Hence, mixing time T is defined as minimum length of random walk required to reach a stationary distribution and it is parameterized by a variation distance parameter $\epsilon$ (\ref{eqn:mt}).  
%
%\begin{equation} \label{eqn:mt}
%T(\epsilon) = max_i min\{t:|\pi - \pi^{(i)}P^t|_1 < \epsilon\} 
%%\text{Where T is mixing time of markov chain parameterized by \epsilon. \pi is the stationary distribution, \pi^i is the initial distribution, P^t is transition matrix ap t steps and |.|_1 is the total variation distance }
%\end{equation}
%
%Now to establish bounds on the mixing time for graph G, we used the second largest Eigenvalue method (\ref{eqn:slem}). If P is the transition matrix of graph G (as decribed in \cref{eqn:mt} ), and ${\lambda}_i$ for $1\leq i \leq n$ are the eigenvalues of P, such that they are labelled in decreasing order i.e. $1 = \lambda_1 > \lambda_2 \geq \lambda_3 ... \geq \lambda_n > -1$, then second largest eigenvalue $\mu$ is defined as $\mu = max(|\lambda_2|, |\lambda_{n-1}|)$. And the mixing time $T(\epsilon)$ is bounded as equation \ref{eqn:slem}.
%
%\begin{equation} \label{eqn:slem}
%\frac{\mu}{2(1-\mu)}log(1/2\epsilon)\leq T(\epsilon) \leq \frac{log(n) + log (1/\epsilon)}{1-\mu}
%\end{equation}
%
%\paragraph{Methodology}
%To measure the mixing time and establish bounds on the same for our ripple network, we took the undirected biggest component of whole network (as in section \ref{}), say graph G and found its corresponding transition matrix P (as described above). Then we directly calculated the second largest eigenvalue $\mu$ (As described above). Then using equation \ref{eqn:slem}, we established the lower bound on mixing time, as represented in Figure~\ref{figure:mt}.
%
%We check the mixing time of network by removing all the lower degree nodes in network. To do so, we iteratively removed all the nodes with degree 1. But we observed that from second iteration onwards, we did not get any significant change in graph. Hence, we only found the bounds for ripple network with single degree nodes removed (figure \ref{figure:mt})
%\begin{figure}
%\includegraphics[height=\columnwidth, angle=270]{images/mixing-1.eps}
%\caption{Lower bound on mixing time for ripple network (represented by ripple) and ripple network by removing nodes with degree 1 (represented by ripple 1)
%\TODOA{reduce the figure height. Better captions}
%\label{figure:mt}}
%\end{figure}
%
%\paragraph{Results}
%As we observe from Figure~\ref{figure:mt}, the lower bound on the mixing time for a given variation distance $\epsilon$ is large. For example, for $\epsilon = 0.1$, the mixing time was around 280, which means even for a variation of 0.1, we need to take a random walk of length of around 280 to reach a stationary distribution. Hence, the network appears to be ``slow mixing'' \TODON{More implications ??}.
%
%When we prune and remove the single degree node, we see that there is a significant improvement in the mixing time. For example, for $\epsilon = 0.1$, mixing time of ripple is 280 while for ripple 1, it is around 120.\TODON{More implications ??}.

==> motif-discussion.tex <==
% !TEX root = main.tex
\section{Motifs}

In non-zero balance links graph, motifs appearing in order are:
69.6\%
\begin{center}
\begin{tikzpicture}[->,shorten >=3pt,auto, thick]
\node[draw, fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (1) {G};
\node[draw,xshift=2cm,fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (2) {U};
\node[draw,xshift=-2cm, fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (3) {U};
\path (1.east) edge (2.west);
\path (1.west) edge (3.east);
\end{tikzpicture}
\end{center}

12.5\%
\begin{center}
\begin{tikzpicture}[->,shorten >=3pt,auto, thick]
\node[draw, fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (1) {G};
\node[draw,xshift=2cm,fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (2) {MM};
\node[draw,xshift=-2cm, fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (3) {U};
\path (1.east) edge (2.west);
\path (1.west) edge (3.east);
\end{tikzpicture}
\end{center}

11.8\%
\begin{center}
\begin{tikzpicture}[->,shorten >=3pt,auto, thick]
\node[draw, fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (1) {U};
\node[draw,xshift=2cm,fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (2) {U};
\node[draw,xshift=-2cm, fill=white,circle,inner sep=2pt, text width=0.5cm, align=center] (3) {U};
\path (1.east) edge (2.west);
\path (1.west) edge (3.east);
\end{tikzpicture}
\end{center}

note - An issue with the graph with all links - not able to get output with algorithm



==> security-availability.tex <==
% !TEX root = main.tex

\section{Security of credit in Ripple}
\label{sec:sec-avail-ripple}

In this section, we analyze the security of the credit in the \nw from different angles. 
First, we study the effect of \emph{unexpected credit balance shifts} due to 
misuse of the rippling operation by users and 
show how it affects to the credit from \accs in the \nw. 
Second, we investigate the \emph{resilience} of the \nw 
to gateways improperly using the rippling functionality, impeding other \accs from 
using their credit. We investigate the \payroutes gateway as a real case study 
of this problem. Finally, we study the effect of 
\emph{stale exchange offers} available in the \nw and how users in the \nw are 
affected by them.

%We stress that the observations we describe in this section are only based on 
%\emph{valid and necessary} operations included in the \nw definition rather than 
%exploiting a weakness in the Ripple protocol (e.g., leverage a leaked secret key). 
%Therefore, we believe that more education is required for Ripple \users for how to 
%use the credit associated to their Ripple \accs. 


==> xrp-distribution.tex <==
% !TEX root = main.tex
\section{XRP tokens distribution}
%\begin{figure}[b]
%\centering
%\includegraphics[height=0.9\columnwidth]{images/xrpbalPerYear.PNG}
%\caption{XRP tokens distribution.\label{fig:XrpTokenDistribution}}
%\end{figure}

\TODOP{We will drop this in the end if we do not find a place for it in the body of the paper}

At the beginning, 99,994,523,265 XRP tokens were mined. As per October 2017, 38,343,841,883 XRP tokens are in circulation in market. The owners of Ripple are planning to hold $30\%$ of total tokens with them and rest of the tokens are released every month at rate of 1 billion. In terms of market cap, XRP is worth 8,784,190,737 USD and stands 4th as of date after Bitcoin, Ethereum and Bitcoin Cash. We study the distribution of XRP tokens since its inception. We observed a tree structure in XRP distribution where the root node sends XRP tokens in bulk to its children, who in turn creates chunks of these tokens and forward them to their respective children. We denote root as "Tier 0" node, its children as ``Tier 1'' nodes and so on. We denote a node with nickname ``X.distributor.1'' as ``Tier 0'' node as it held all XRP tokens in the beginning, activated 9 XRP accounts on 26th Jan, 2013 and transferred minimum 8 billion tokens in each of them. The naming convention of each of these 9 accounts is ``X.FortKnox.i'' where $i = 2, \cdots, 9, a$. All ``FortKnox'' nodes are ``Tier 2'' nodes which further activated another XRP accounts (i.e., Tier 3) and distributed XRP tokens amongst them.  

